ARTEMIS: Neutralizing BGP Hijacking within a Minute

BGP prefix hijacking is a critical threat to Internet organizations and users. Despite the availability of several defense approaches (ranging from RPKI to popular third-party services), none of them solves the problem adequately in practice. In fact, they suffer from: (i) lack of detection comprehensiveness, allowing sophisticated attackers to evade detection, (ii) limited accuracy, especially in the case of third-party detection, (iii) delayed verification and mitigation of incidents, reaching up to days, and (iv) lack of privacy and of flexibility in post-hijack counteractions, on the side of network operators. In this work, we propose ARTEMIS (Automatic and Real-Time dEtection and MItigation System), a defense approach (a) based on accurate and fast detection operated by the AS itself, leveraging the pervasiveness of publicly available BGP monitoring services and their recent shift towards real-time streaming, thus (b) enabling flexible and fast mitigation of hijacking events. Compared to previous work, our approach combines characteristics desirable to network operators such as comprehensiveness, accuracy, speed, privacy, and flexibility. Finally, we show through real-world experiments that, with the ARTEMIS approach, prefix hijacking can be neutralized within a minute.

==> Discussion.tex <==
\myitem{Coexistence of ARTEMIS with RPKI.} 
\blues{In a world with 100\% successful and error-free deployment of RPKI~\cite{rpki-rfc} and BGPsec~\cite{bgpsec-specification-2015}, most hijacking attacks would not be effective. However, this is far from reality~\cite{rpki-monitor,RiPKI-hotnets-2015,RPKI-deployment-2016}, and networks need solutions that can work today and be able to co-exist with RPKI. \artemis is immediately deployable (as our prototype shows), does not interfere with RPKI (\eg de-aggregated prefixes and ASNs of outsourcing organizations can be added to ROAs), and could even be used in cooperation with RPKI (\eg updating or verifying the RPKI database).
}

%\blues{In a world with 100\% successful and error-free deployment of secure BGP and RPKI, the ARTEMIS approach would be obsolete, since it could be fully replaced by strong and verifiable cryptographic mechanisms.
%However, since this world seems to be very far in the future~\cite{rpki-monitor,RiPKI-hotnets-2015,RPKI-deployment-2016}, networks still require solutions which can work today, while being able to co-exist and ideally
%cooperate with the partial deployments of RPKI. While not a core requirement of the system, ARTEMIS could e.g., capitalize on ROV to detect type-N hijacks more accurately, if it is configured with the valid ROA certificates that the operator deploying ARTEMIS is using. Moreover, ARTEMIS (with the permission of the operator) and public RPKI registries could benefit from each other by exchanging data on (in)valid routes and suspected hijacks, thus verifying the accuracy of the RPKI database and the ARTEMIS detection mechanisms.
%}


\myitem{Modular/extendable system design.} 
\blues{The \artemis design is modular and configurable, thus fitting the needs of the operators and being amenable to future extensions. This allows operators/researchers to add or modify modules on demand, without affecting the functionality of the entire system. For instance, the more challenging task of detecting Type-N, $N\geq2$, hijacking attacks, could be enriched with data-analytics or machine-learning approaches, e.g.,~\cite{caida-hijacks-project,snas-io}, or new control-plane information sources, such as the recently introduced BMP protocol~\cite{scudder2016bgp}. Moreover, \artemis can be enhanced with detection/mitigation modules against attackers beyond the adopted threat model (\ie hijackers controlling multiple ASes \ed{and launching Type-N, $N\geq2$, attacks--pavlos}).
}

%\blues{The mechanisms which comprise the detection sub-system of ARTEMIS (see Section~\ref{sec:detection}), can operate in sequence (such as the Stage 1 and Stage 2 mechanisms for the detection of type-N hijacks in Section~\ref{sec:detection-types-N}), or in parallel, such as the checks for sub-prefix, type-0/1 or type-N hijacks. In general, the design of this sub-system if highly modular; the main concept is to be able to add new modules on demand and form pipelines with pre-existing ones, in order to enhance the accuracy and efficiency of the detection process (e.g., by reducing false positives). 
%%These pipelines, as well as the parallelization of the system, can be tuned/configured by the network operator depending on his preferences. 
%For example, Stage 2 might be chosen as an optional verification stage or be accompanied/replaced by a new mechanism relying on BGP route poisoning~\cite{}.


%\myitem{Implementation of Outsourcing BGP Announcements.} 
\myitem{Outsourcing BGP announcements in practice.} 
\blues{The implementation of the proposed outsourcing hijacking mitigation mechanism can be based on practices already undertaken by DDoS security organizations as described in Section~\ref{sec:mitigation-techniques}. In particular, the outsourcing organization is automatically informed by ARTEMIS about an ongoing hijack, and is authorized (in advance) by the victim AS to announce the affected prefix(es). Afterwards, a tunnel (\eg GRE-based) between the outsourcing organization and the victim AS can be activated to relay the attracted traffic to the victim (\eg similarly to~\cite{Peter-One-Tunnel-Sigcomm-2014}). We are investigating such automated protocols and tunnel setups over a popular SDN platform as well~\cite{artemis-onos-wiki}.
}
%\blues{The implementation of this outsourcing mitigation mechanism can be based on practices already undertaken by DDoS security organizations as described in Section~\ref{sec:mitigation-techniques}. In particular, it could be based on a paid-service model where the outsourcing provider is informed automatically by ARTEMIS on an ongoing hijack, and is authorized by the victim AS to announce the affected prefix(es) from its own AS. The protocol for such a reaction could be pre-configured upon the start of the outsourcing relationship. Afterwards, a tunnel (e.g., GRE-based) between the outsourcing provider and the victim AS (or its direct provider, if no IP tunnel endpoints in the victim itself are available during the hijack) is used to relay the attracted traffic to the legitimate announcer; the tunnel can be pre-configured for efficiency, and be activated only in the case of attack. In fact, we are investigating such automated protocols and tunnel setups in a parallel thread of development of ARTEMIS over popular SDN platforms~\cite{artemis-onos-wiki}, enabling the automation of multi-domain orchestration.
%}



\myitem{Alerts and monitoring under duress.}
\blues{The communication between the victim AS and the monitoring services (and/or an outsourcing organization) might be interrupted in extended hijacking attacks (\eg when all the owned prefixes are hijacked). To prevent this, an AS can run \artemis as a cloud service (\ie outside its network): if a notification about a hijack cannot reach the system of the victim AS through an IP-level connection, then an ``out-of-band'' (\eg cellular network) notification can take place.
}
%\blues{In case a legitimate AS is hijacked, its IP-level connection to the monitoring services might be interrupted, and thus it will never receive information about illegitimate paths and hijack attempts. To prevent this, the legitimate AS can run the ARTEMIS detection process as a cloud service, and if a notification about a hijack cannot reach the system within the legitimate AS, then an ``out-of-band'' notification takes place. Such a mechanism could be based on SMS notifications via the cellular network or other non-IP channels (e.g., telephone).
%}


==> Preliminaries.tex <==
%This section provides the necessary background on BGP prefix hijacking attacks and defences, and discusses the shortcomings of current practices that motivate our research. We first present the considered threat model that describes how a hijacking attack can take place and its characteristics (Section~\ref{sec:hijack-types-characteristics}). Then we discuss why hijacking remains -even today- a serious threat for the Internet and is not efficiently resolved by existing approaches (Section~\ref{sec:motivation})


==> Survey.tex <==

%\subsection{Methodology / questions}
%\subsection{Most interesting results}

To increase our understanding of existing BGP hijacking defenses and the needs of network operators, we launched a survey on mailing lists such as NANOG and RIPE)~\cite{google-survey-hijacking}. The survey is anonymous and comprises 21 questions studying (a) the operators' awareness of BGP prefix hijacking attacks, (b) presently used defenses (if any) against BGP prefix hijacking, (c) the willingness to adopt new defense mechanisms, and (d) reasons that may hinder the deployment of BGP prefix hijacking defenses.  

We received answers from \red{75} participants operating \red{(from different positions; Fig.~\ref{fig:survey-q4})} a broad variety of networks (ISPs, CDNs, IXPs, etc.\red{; Fig.~\ref{fig:survey-q1}}) all over the world (\red{Fig.~\ref{fig:survey-q2}}).


\subsection{Impact of Hijacks}\label{sec:survey-impact}


\textbf{BGP prefix hijacking is a real threat and concerns network operators.} \red{More than half} of the operators testified that their organization has been victim of a hijack in the past \red{(Fig.~\ref{fig:survey-q9})}. However, the vast majority is concerned about BGP prefix hijacking in the Internet \red{(Fig.~\ref{fig:survey-q6})} and their own networks \red{(Fig.~\ref{fig:survey-q7})}.

\textbf{Hijacks have a severe and lasting impact.} Operators evaluate the impact of a potential hijack for their network (in terms of \textit{duration} and \textit{number of disrupted services}) as shown in \red{Table~\ref{table:survey-impact}}: (i) the vast majority (\red{76\%}) expects the impact of the hijack to last for a long time (few hours or more), while (ii) opinions are divided on whether the hijack will affect a few or many of their services/clients, which indicates that there are concerns both for extended (e.g., route leaks) and limited (e.g., malicious attacks) hijacks. Moreover, their past experience \red{(Fig.~\ref{fig:survey-q10})} shows that most hijacks lasted long: more than \red{57\%} of hijacks lasted more than an hour, and \red{25\%} lasted \textit{more than a day}; around \red{28\%} are short-term hijacks, lasting a few minutes (\red{14.3\%}) or a few seconds (\red{14.3\%}).

\begin{table}
\centering
\caption{Question 8: How severe do you consider the potential impact of a BGP prefix hijacking against your network?}
%\label{table:survey-q8}
\label{table:survey-impact}
\begin{tabular}{c|ccc}
{}& {no impact}& {$\sim$ minutes}& {$\sim$ hours}\\
\hline
{few services/clients}& {0\%}& {~9.3\%}& {28.0\%}\\
{many services/clients}& {0\%}& {~9.3\%}& {48.0\%}
\end{tabular}
\end{table}


\begin{figure}
\centering
\subfigure[]{\includegraphics[width = 0.43\linewidth]{./figures/fig_survey_how_concerned_TEMP}}
\subfigure[]{\includegraphics[width = 0.49\linewidth]{./figures/fig_survey_how_likely_TEMP}}
\caption{(a) How concerned are you about BGP prefix hijacking incidents on the Internet? (b) How likely do you consider that your network will be a victim of a BGP prefix hijacking incident in the future?}
\label{fig:survey-concern}
\end{figure}




\subsection{Defences against Hijacks}\label{sec:survey-defences}

\textbf{RPKI deployment is limited.} In accordance with previous studies~\cite{RPKI-deployment-2016}, most of the network operators (\red{71\%}) answered that their networks have not deployed RPKI \red{(Fig.~\ref{fig:survey-q11})}. There are various reasons for this as shown in \red{Fig.~\ref{fig:survey-q12}}: mainly due to its \textit{limited adoption} and \textit{little security benefits}, but also due to the increased \textit{CAPEX and OPEX costs}, and increased \textit{complexity} and \textit{processing} issues. 

\textbf{Practical defences comprise route filtering, anycasting, and de-aggregation.} The responses to the (optional) question what other mechanisms that relate to the defence of BGP prefix hijacking are used by networks are shown in Fig.~\ref{fig:survey-q14}. The majority of the participants (among those who provided answers for this optional question), \red{17 networks}, use \textit{route filtering} as a proactive defence to protect their and their customers' prefixes from being hijacked. \textbf{Route filtering} is implemented in various ways (based on their answers) including for example: prefix origin (e.g., from IRR records) or AS-path filtering; filtering at edge routers (with customers/peers) or route servers (IXPs). Less popular approaches are \textit{anycast} \red{(2 answers)} and \textit{deaggregation} \red{(4 answers)}. Finally, \red{5} operators (from CDNs or tier-1 networks) mention that they peer with many other networks, which helps them protect their networks from hijacking events (i.e., by reducing their impact).
%
%We define as \textbf{anycast}, in terms of BGP hijacking, the approach where a network announces its prefixes through different locations to its neighbors (e.g., by setting up or enabling unused/backup links)\footnote{Only one network operator used the word ``anycast'' to describe this type of defence. Other answers for this type of defence, describe it as, e.g., 
%\begin{itemize}
%\item ``Adjacencies with most default-free networks to help limit the scope of a potential hijacking.''
%\item ``100s of BGP sessions around the globe allowing us to essentially hijack back.''
%\item ``We directly peer with as many important networks as possible.''
%\item ``Extremely high peering and thus most of larger networks have direct path to us and will likely avoid anyone else announcing same pool from their ASN.''
%\end{itemize}
%}. 
%Some examples of the received answers which we classify as ``anycast'' are: after a prefix hijack is detected, a network operator enables ``100s of BGP sessions around the globe, to essentially hijack back'' (reactive approach); or, two networks establish adjacencies (``extremely high peering'') to limit the effects of potential hijacks, due to direct paths to these peers (proactive approach). Finally, \textbf{prefix deaggregation} is a reactive approach where a network, upon receiving a hijack alert, announces (usually manually; only one operator mentions that they implement an automatic de-aggregation mechanism) sub-prefix of the hijacked prefix. As a result, networks having received the bogus route (from the hijacker), when receive the routes for the sub-prefixes (from the legitimate AS), re-route to the legitimate AS due to the more specific prefix preference.


\subsection{Detection and Mitigation of Hijacks.}

\textbf{Hijack detection mainly relies on third parties.} The majority of networks \red{(61.3\%)} use a third party detection service, which notifies them for hijacking incidents against their prefixes \red{(see Fig.~\ref{fig:survey-q15})}. BGPmon is the most popular detection service, \red{see Fig~\ref{fig:survey-q16}}. The satisfaction of operators from third parties varies a lot; some use them because they are satisfied and some other because there are no alternatives (and it is not possible to develop their own detection service
\footnote{This variation of answers can be seen in the following examples from the detailed answers in our survey:
\begin{itemize}
\item ``pretty happy with it'', ``no issues so far'', ``it works fine [..], but is relatively limited'', ``I hate it'', ``It's ok'', `` it seems to work quite well the few times I have needed it'', ``Better than nothing, but a lot of false alerts'', ``It rules!'', ``It is very noisy because it does not know a damn thing about IXP route servers'', ``Not great''
\end{itemize}
}. Moreover, \red{17.3\%} of networks also rely on third parties, since they expect to get notified for a hijack by receiving notification from colleagues, clients, mailing lists, etc. In total, \red{61.3+17.3=78.6\%} of the networks rely on third parties for the detection of hijacks against their prefixes. \red{About one third} of the networks have deployed a local hijack detection mechanism (e.g., by monitoring the disruption of their services)\footnote{Among the ``other'' answers, a high percentage of answers relates to the observation of -or, reception of complaints about- disruption in their services.}. Finally, a significant percentage \red{8\%} probably would not (does not know if would) learn about a hijack. 

\textbf{Mitigating through de-aggregation and contacting other networks.} \blue{[In this question, we provided the answers; People could answer in a different way if it was an open question]} Asking operators what would be the countermeasures they would take to mitigate a prefix hijacking, the majority \red{(62.7\%; see Fig.~\ref{fig:survey-q17})} responded that would announce more specific prefixes and contact the offending network (i.e., hijacker) or its providers. \red{5.3\%} would follow \textit{only} the former approach (de-aggregation) and \red{25.3\%} \textit{only} the latter (contact other operators). This indicates that although de-aggregation is not widely used currently \red{(see Fig.~\ref{fig:survey-q14})}, operators find it a good solution and are willing to proceed to such actions after a hijacking event.


 

\subsection{New Mitigation Mechanisms}
We ask network operators about their willingness to deploy new mitigation mechanisms, as well as what are the desired characteristics.


The main practices that networks currently use for hijack mitigation are prefix de-aggregation, contacting other networks, and anycasting \red{(see Figs.~\ref{fig:survey-q14} and~\ref{fig:survey-q17})}. Since the above approaches have some shortcoming, e.g, deaggregation is not efficient when a /24 prefix is hijacked, contact of network operators and/or anycasting is usually done manually and thus add significant delay, we ask the network operators about their willingness to deploy new mitigation mechanisms, as well as what are the desired characteristics.

We first ask them about their willingness to outsource functions, in order to enhance their defence against hijacks. Outsourcing can be very efficient as we show in Sec.~\ref{}. However, \red{61\%} of the operators are not willing to outsource their defence to hijacks (Fig.~\ref{fig:survey-q18}). This shows that a potential mechanism should not be entirely based on collaboration or outsourcing, since this would not be acceptable by many networks. To this end, the approach we propose is flexible and can be operated in two modes: self-operated and outsourced. On the other hand, a significant percentage \red{39\%} does not reject the possibility to outsource such functions.

The reasons for their reluctance to outsource are given in \red{Fig.~\ref{fig:survey-q19}}, where it can be seen that the cost and the need to share private information about their network are the main factors. Administrative and technical overhead may also prevent outsourcing. This is a first indication about the characteristics of a future outsourcing system: low cost, privacy preserving, and easy to operate.

More specific results about what would be the information/control that they would \textit{not} be willing to share/allow with an outsourcing organization, are given in Fig.~\ref{fig:survey-q20}. As it can be seen, most of them are willing to share information about their prefixes and AS-neighbors \red{(95\%)}, as well as their routing policies \red{(80\%)}. A smaller percentage would allow BGP announcements to be controlled or done from the outsourcing organization.



Finally, the importance (according to operators) of different characteristics that a mitigation system should have, is shown in Table~\ref{table:survey-q21} (ranked with higher importance). A graphical representation of the importance of these characteristics for the network operators is given in \red{Fig.~\ref{fig:survey-q21}}, where the rightmost characteristics are considered of higher importance.


\subsection{ALL SURVEY PLOTS}

\begin{figure*}
\centering
\subfigure[Q1]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_type_of_organization}\label{fig:survey-q1}}
\subfigure[Q2]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_continent}\label{fig:survey-q2}}
\subfigure[Q4]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_position_in_company}\label{fig:survey-q4}}
\subfigure[Q5]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_know_BGP}\label{fig:survey-q5}}
\subfigure[Q6]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_concerned_BGP}\label{fig:survey-q6}}
\subfigure[Q7]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_concerned_BGP_your_network}\label{fig:survey-q7}}
\subfigure[Q9]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_past_victim}\label{fig:survey-q9}}
\subfigure[Q10]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_how_long_affected}\label{fig:survey-q10}}
\subfigure[Q11]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_use_RPKI}\label{fig:survey-q11}}
\subfigure[Q12]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_reasons_rpki}\label{fig:survey-q12}}
\subfigure[Q13]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_use_defence_other_RPKI}\label{fig:survey-q13}}
\subfigure[Q14]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_what_defence_other_RPKI}\label{fig:survey-q14}}
\subfigure[Q15]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_notification}\label{fig:survey-q15}}
\subfigure[Q16]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_what_detection_service}\label{fig:survey-q16}}
\subfigure[Q17]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_mitigation}\label{fig:survey-q17}}
\subfigure[Q18]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_outsource}\label{fig:survey-q18}}
\subfigure[Q19]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_factors_not_outsource}\label{fig:survey-q19}}
\subfigure[Q20]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_not_share_with_outsource}\label{fig:survey-q20}}
\subfigure[Q21]{\includegraphics[width = 0.24\linewidth]{./figures/fig_survey_important_factors_mitigation}\label{fig:survey-q21}}
\caption{Survey results.}
\end{figure*}


\begin{itemize}
\item Question 1: Which term(s) would best characterize your organization?
\item Question 2: In which continent(s) does your company operate?
\item Question 4: What is your position in your company?
\item Question 5: Do you know what BGP prefix hijacking is and how it can happen?
\item Question 6: How concerned are you about BGP prefix hijacking incidents on the Internet?
\item Question 7: Are you concerned that your network may be a victim of a BGP prefix hijacking incident in the future?
\item Question 9: Has your organization been a victim of a BGP prefix hijacking incident in the past?
\item Question 10: If your organization was a victim of a BGP prefix hijacking incident, for how long was your network affected?
\item Question 11: Do you use RPKI in your network?
\item Question 12: If no, what are the main reasons for not using RPKI?
\item Question 13: Do you use in your network any other defense mechanisms (other than RPKI) that protect your/others' prefixes from BGP prefix hijacking?
\item Question 14: If yes, what mechanisms do you use? Could you provide a brief description? Open question/answers
\item Question 15: In your network, how would you learn about a hijacking incident against your prefix(es)?
\item Question 16: If you use a local or third-party detection service or system, could you please give us more details about it? Open question
\item Question 17: How would you mitigate a hijack against your prefixes if you were notified about an on-going event?
\item Question 18: Would you outsource functions relating to the detection and mitigation of prefix hijacking incidents to a third-party, if this helps your organization reduce its risks?
\item Question 19: If no, what are the main factors that would affect your decision not to outsource prefix hijacking mitigation? [check max 2 factors] (optional) 
\item Question 20: Assuming you fully trust an outsourcing organization for prefix hijacking mitigation, what is the information/control (if any) you are still NOT willing to share/allow?
\item Question 21: How important do you consider the following characteristics for the deployment of a new defense system in your network?
\end{itemize}


%
%\begin{table}
%\centering
%\caption{Question 8: How severe do you consider the potential impact of a BGP prefix hijacking against your network?}
%\label{table:survey-q8}
%\begin{tabular}{c|ccc}
%{}& {no impact}& {~minutes}& {~hours}\\
%\hline
%{few services/clients}& {0\%}& {11.9\%}& {32.2\%}\\
%{many services/clients}& {0\%}& {8.5\%}& {40.7\%}
%\end{tabular}
%\end{table}

\begin{table}
\centering
\caption{Question 21: How important do you consider the following characteristics for the deployment of a new defense system in your network?}
\label{table:survey-q21}
\begin{small}
\begin{tabular}{c|cccc}
{Importance (0: Low ... 3:High)}& {0}& {1}& {2}& {3}\\
\hline
{Effectiveness of mitigation}				& {~0~~\%}& {~2.7\%}& {49.3\%}& {48.0\%}\\
{Fast mitigation}							& {~2.7\%}& {14.7\%}& {38.7\%}& {44.0\%}\\
{Self-managed/operated}						& {~1.3\%}& {18.7\%}& {38.7\%}& {41.3\%}\\
{Ease of operating/troubleshooting}			& {~0~~\%}& {21.3\%}& {40.0\%}& {38.7\%}\\
{Low cost}									& {~6.7\%}& {17.3\%}& {52.0\%}& {24.0\%}\\
{Ease of installation}						& {~1.3\%}& {30.7\%}& {53.3\%}& {14.7\%}\\
{Minimum changes to network configuration}	& {~5.3\%}& {26.7\%}& {49.3\%}& {18.7\%}\\
{Low false positives (detection)}			& {~2.7\%}& {12.0\%}& {29.3\%}& {41.3\%}\\
{Privacy (e.g., routing policies)}			& {~8.0\%}& {32.0\%}& {32.0\%}& {28.0\%}\\
{Low false negatives (detection)}			& {~1.3\%}& {13.3\%}& {36.0\%}& {34.7\%}\\
\end{tabular}
\end{small}
\end{table}

%
%%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_continent}
%\caption{Question 2: In which continent(s) does your company operate?}
%\label{fig:survey-q2}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_position_in_company}
%\caption{Question 4: What is your position in your company?}
%\label{fig:survey-q4}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_know_BGP}
%\caption{Question 5: Do you know what BGP prefix hijacking is and how it can happen?}
%\label{fig:survey-q5}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_concerned_BGP}
%\caption{Question 6: How concerned are you about BGP prefix hijacking incidents on the Internet?}
%\label{fig:survey-q6}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_concerned_BGP_your_network}
%\caption{Question 7: Are you concerned that your network may be a victim of a BGP prefix hijacking incident in the future?}
%\label{fig:survey-q7}
%\end{figure}
%
%
%
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_past_victim}
%\caption{Question 9: Has your organization been a victim of a BGP prefix hijacking incident in the past?}
%\label{fig:survey-q9}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_how_long_affected}
%\caption{Question 10: If your organization was a victim of a BGP prefix hijacking incident, for how long was your network affected?}
%\label{fig:survey-q10}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_use_RPKI}
%\caption{Question 11: Do you use RPKI in your network?}
%\label{fig:survey-q11}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_reasons_rpki}
%\caption{Question 12: If no, what are the main reasons for not using RPKI?}
%\label{fig:survey-q12}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_use_defence_other_RPKI}
%\caption{Question 13: Do you use in your network any other defense mechanisms (other than RPKI) that protect your/others' prefixes from BGP prefix hijacking?}
%\label{fig:survey-q13}
%\end{figure}
%
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_what_defence_other_RPKI}
%\caption{Question 14: If yes, what mechanisms do you use? Could you provide a brief description? Open question/answers}
%\label{fig:survey-q14}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_notification}
%\caption{Question 15: In your network, how would you learn about a hijacking incident against your prefix(es)?}
%\label{fig:survey-q15}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_what_defence_other_RPKI}
%\caption{Question 16: If you use a local or third-party detection service or system, could you please give us more details about it? Open question}
%\label{fig:survey-q16}
%\end{figure}
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_mitigation}
%\caption{Question 17: How would you mitigate a hijack against your prefixes if you were notified about an on-going event?}
%\label{fig:survey-q17}
%\end{figure}
%
%
%\begin{figure}
%\includegraphics[width = \linewidth]{./figures/fig_survey_outsource}
%\caption{Question 18: Would you outsource functions relating to the detection and mitigation of prefix hijacking incidents to a third-party, if this helps your organization reduce its risks?}
%\label{fig:survey-q18}
%\end{figure}
%
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_factors_not_outsource}
%\caption{Question 19: If no, what are the main factors that would affect your decision not to outsource prefix hijacking mitigation? [check max 2 factors] (optional) }
%\label{fig:survey-q19}
%\end{figure}
%
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_not_share_with_outsource}
%\caption{Question 20: Assuming you fully trust an outsourcing organization for prefix hijacking mitigation, what is the information/control (if any) you are still NOT willing to share/allow?}
%\label{fig:survey-q20}
%\end{figure}
%
%
%
%\begin{figure}
%\centering
%\includegraphics[width = \linewidth]{./figures/fig_survey_important_factors_mitigation}
%\caption{Question 21: How important do you consider the following characteristics for the deployment of a new defense system in your network? }
%\label{fig:survey-q21}
%\end{figure}
%

